The role of Blockchain in DDoS attacks mitigation: techniques, open challenges and future directions

With the proliferation of new technologies such as Internet of Things (IOT) and Software-Defined Networking(SDN) in the recent years, the distributed denial of service (DDoS)attack vector has broadened and opened new opportunities for more sophisticated DDoS attacks on the targeted victims. The new attack vector includes unsecured and vulnerable IoT devices connected to the internet, denial of service vulnerabilities like southbound channel saturation in the SDN architecture. Given the high-volume and pervasive nature of these attacks, it is beneficial for stakeholders to collaborate in detecting and mitigating the denial of service attacks in a timely manner. The blockchain technology is considered to improve the security aspects owing to the decentralized design, secured distributed storage and privacy. A thorough exploration and classification of blockchain techniques used for DDoS attack mitigation is not explored in the prior art. This paper reviews and categorizes the existed state-of-the-art DDoS mitigation solutions based on blockchain technology. The DDoS mitigation techniques are classified based on the solution deployment location i.e. network based, near attacker location, near victim location and hybrid solutions in the network architecture with emphasis on the IoT and SDN architectures. Additionally, based on our study, the research challenges and future directions to implement the blockchain based DDoS mitigation solutions are discussed. We believe that this paper could serve as a starting point and reference resource for future researchers working on denial of service attacks detection and mitigation using blockchain technology.

==> 3relatedwork.tex <==
\section{RELATED WORK}
\label{sec:relatedwork}

Technologies such as machine learning (ML), blockchain, internet of things (IoT), and software defined networking (SDN) are well suited to improve the security in digital world but also exhibit new security concerns and issues \cite{Lin2017AChallenges} \cite{Ahmad2019AThings} \cite{Muthanna2019} \cite{Wang2019TheSurvey}\cite{Gao2018SecurityNetworks}\cite{Boppana2020AnalyzingNetworks}\cite{Qu2018}\cite{DantasSilva2020}\cite{Dwivedi2019}\cite{Rathore2019}. Some researchers also used combinations of these technologies to address security challenges  ranging from malware analysis, Domain Name System (DNS) Security, to network security as well as privacy issues \cite{Hussain2020MachineChallenges} \cite{daCosta2019InternetApproaches} \cite{Dong2019AEnvironments}\cite{Liu2020ALearning} \cite{Elagin2020}. Our focus in this paper is specific to DDoS-attack detection and mitigation techniques in conventional networks, software defined networks, cloud environments and internet of things \cite{Srivastava20AMechanisms} \cite{Dong2019AEnvironments} \cite{BeslinPajila2020DetectionSurvey} \cite{Sonar2014AThings} \cite{Park2017}. The currently known techniques include machine learning or deep learning (ML/DL) algorithms to classify the attacks, anomaly-based detection, and signature-based detection.

A recent advancement in peer to peer networks with blockchain technology enabled utilization of  decentralized network concepts for multiple application areas like finance, healthcare, real estate, supply chain management, security \cite{BlockchainInsider}. Although blockchain mainly provides the anonymity, privacy and secured data storage in security applications,  researchers also explored the applicability of blockchain technology in DDoS attack information sharing, threat intelligence information sharing to quickly respond to the DDoS attacks. Singh et al.  \cite{Singh2020UtilizationAttacks} present a survey of DDoS mitigation techniques using blockchain technology. The authors considered four known blockchain based DDoS mitigation approaches for comparison; highlighted the operation of these mitigation mechanisms and assessed  the practical applicability of these implementations \cite{Rodrigues2017AContracts} \cite{BurgerZurich2017CollaborativeBlockchains} \cite{Javaid2018MitigatingBlockchain}\cite{Kataoka2018TrustSDN}. Wani et al. \cite{Wani2021} discussed the prior art distributed denial of service attack mitigation using blockchain by describing the methodology on how the related papers are collected and proposing the taxonomy based on the technologies like artificial intelligence, information sharing capability and blockchain types. However, a comprehensive and systematic review of the state-of-the-art work with classification based on the solution implementation location by leveraging the blockchain technology to detect and mitigate the DDoS attacks in digital world and also detail description of DDoS attacks targeting Blockchain platforms to protect decentralized networks is not covered in the prior art. Our motivation for this work is to bridge the knowledge gap between network security researchers and the blockchain developing community and enable the researchers to access this article as a reference point to continue the research of using blockchain technology in network security.

